Conditional Generative Refinement Adversarial Networks for Unbalanced Medical Image Semantic Segmentation

We propose a new generative adversarial architecture to mitigate imbalance data problem in medical image semantic segmentation where the majority of pixels belongs to a healthy region and few belong to lesion or non-health region. A model trained with imbalanced data tends to bias toward healthy data which is not desired in clinical applications and predicted outputs by these networks have high precision and low sensitivity. We propose a new conditional generative refinement network with three components: a generative, a discriminative, and a refinement network to mitigate unbalanced data problem through ensemble learning. The generative network learns to a segment at the pixel level by getting feedback from the discriminative network according to the true positive and true negative maps. On the other hand, the refinement network learns to predict the false positive and the false negative masks produced by the generative network that has significant value, especially in medical application. The final semantic segmentation masks are then composed by the output of the three networks. The proposed architecture shows state-of-the-art results on LiTS-2017 for liver lesion segmentation, and two microscopic cell segmentation datasets MDA231, PhC-HeLa. We have achieved competitive results on BraTS-2017 for brain tumour segmentation.

==> chapters/abstract.tex <==
\begin{abstract}
We propose a new generative adversarial architecture to mitigate imbalance data problem in medical image semantic segmentation where the majority of pixels are belong to healthy region and few belong to lesion or non-health region. A model trained with imbalanced data tends to bias toward healthy data which is not desired in clinical applications and predicted outputs by these networks have high precision and low sensitivity. We propose a new conditional generative refinement network with three components: a generative, a discriminative, and a refinement network to mitigate unbalanced data problem through ensemble learning. The generative network learns to segment at the pixel level by getting feedback from the discriminative network according to the true positive and true negative maps. On the other hand, the refinement network learns to predict the false positive and the false negative masks produced by the generative network that has significant value especially in medical application. The final semantic segmentation masks are then composed by the output of the three networks. The proposed architecture shows state-of-the-art results on LiTS-2017 for liver lesion segmentation and MDA231 for microscopic cell segmentation. We have achieved competitive results on BraTS-2017 for brain tumour segmentation.
%Finally, we show evidence that the proposed framework is applicable to different types of medical images of varied sizes.
\end{abstract}

==> chapters/relatedwork.tex <==
\section{Related Work} \label{relatedwork}

This section briefs the previous studies carried out in the area of imbalanced dataset learning in medical image analysis~(\ref{imbalanced}-A), and generative adversarial networks in medical image processing~(\ref{GAN}-B) mostly in recent years.


At the datasets level, the objective is to re-balance the class distribution through re-sampling the data space~\cite{kohli2017medical} including SMOTE (Synthetic Minority Over-sampling Technique) of the positive class~\cite{douzas2018effective,mariani2018bagan} or under-sampling of the negative class~\cite{6914453}. %%%%%%%Furthermore, an iterative sampling methodology is used to produce smaller learning sets by removing redundant instances~\cite{morales2012image}.
%%%%%Recently Dong et al.~\cite{dong2018imbalanced} introduced batch-wise mining to tackle with imbalanced of minority class incremental rectification using deep convolutional neural network. 
%In this paper, we apply oversampling including random cropping, rotation, and random scaling region of tumuor(s) as data augmentation in order to balance training data in minority of classes.
%In this paper, we propose a patient-wise batch normalization technique which by enforcing a deep network to maintain both intercluster and inter-class margins.
%our learning algorithm produce inductive bias (learning bias) towards the frequent (majority) and minority of training data, resulting in high performance.
%The motivation behind cost sensitive is to assign a higher cost to less represented set of objects we boost its importance during the learning process. The goal is to minimize the global cost associated with mistake.

The algorithmic based approaches address class imbalanced by modifying learning algorithm to alleviate their bias toward minority class. The most popular approaches are cost sensitive learning where the distribution of the training set is modified with regards to miss-classification costs. The modified distribution is biased towards the costly classes; for example some have focused on balancing with accuracy loss~\cite{sudre2017generalised} and Dice loss~\cite{isensee2017brain,isensee2017automatic}.
%Hashemi et al.~\cite{D11078} proposed asymmetric similarity loss to balance relcall and precision.
\textcolor{red}{It is important to mention that for many clinical dataset it is difficult, time consuming, and expensive to set the actual values in the cost matrix and often they are not given by expert beforehand.
Some approaches address re-balancing through ensemble learning by combining same or different classifiers to improve their generalization ability. The effect of combining redundant ensembles is studied by Sun et al.~\cite{sun2007cost} in terms of the statistical concepts of bias and variance. The predicted results improve in minority class from ensemble combination due to reduction in variance~\cite{sun2007cost}.}
We try to mitigate the negative impact of the class imbalance through ensemble learning from three agents of~\textit{a generative, a discriminative, and a refinement}\textcolor{red}{in way of cost-sensitive approaches}.

%The motivation behind cost sensitive approaches is to assign a higher cost to less represented set of objects we boost its importance during the learning process. We design a cascade architecture and train network in two stages. In first stage generative network in conditional setting learns true positive and true negative of pixels through discriminative network feedback. Hence false positive and false negative have an important impact in a medical application, our algorithm in the second stage is trained on false positive and false negative masks predicted by generator network from the first stage. The final semantic segmentation masks computed by aggregation of two stages output. The goal is to minimize the global cost associated with mistake.

\textbf{A: Imbalanced dataset Learning in Medical Image Analysis:}\label{imbalanced} The class imbalance problem in classification of diseases, abnormal tissues localization or segmentation has been recognized as a significant research problem in recent years and a number of methods have been introduced to improve or mitigate this problem. We can roughly divide the current approaches into two categories: those based datasets level and those approaches on algorithmic level.

At the datasets level, the objective is to re-balance the class distribution through re-sampling the data space~\cite{kohli2017medical} including over sampling of the positive class~\cite{lusa2015joint}, under-sampling of the negative class~\cite{6914453}. Furthermore, an iterative sampling methodology is used to produce smaller learning sets by removing redundant instances~\cite{morales2012image}. Ensemble sampling and hybrid sampling are another solution introduced by Vilches et al.~ \cite{vilches2015contributions}.

The algorithmic based approaches address class imbalanced by ensemble learning; for example training cascade networks in 2D images~\cite{isensee2017brain}, 2.5D images~\cite{wachinger2018deepnat}, 3D images~\cite{kamnitsas2017ensembles}, or hybrid of 2D and 3D images~\cite{isensee2017automatic}.
Since a trained models with unbalanced data, make predictions with high precision and low recall which is undesired in medical routine applications.
Some have focused on balancing recall and precision with asymmetric loss function~\cite{D11078}, or using accuracy~\cite{sudre2017generalised}.
Similar some recent works~\cite{qiu2018nonuniform}, we try to mitigate the negative impact of the class imbalance, with weighted loss function in different formulation.

\textbf{B: Generative Adversarial Networks for Medical Image Analysis:}\label{GAN}The GANs framework in general setting is used for medical image
synthesis~\cite{nie2017medical} in different modalities, cross-domain generation with multi-agent GANs~\cite{guibas2017synthetic}.
%Some researcher applied conditional GANs to find brain tumour or liver tumour location~\cite{}.

Recently, conditional GANs framework used with promising results for abnormal brain tissues segmentation~\cite{rezaei2017conditional}, whole brain segmentation~\cite{Moeskops2017}, and in cascade GANs for whole heart segmentation~\cite{rezaei2018whole}.
Adversarial networks have achieved notable results even on small datasets for prostate cancer detection~\cite{KohlBSYHHRM17}, and mammography mass segmentation~\cite{WentaoZhuX16}.

Unlike previous works~\cite{WentaoZhuX16,KohlBSYHHRM17,Moeskops2017}, we investigate the sequential 2D images into sequential 2D image translation using conditional GAN. 
